A Decomposition-based Approach towards the Control of Boolean Networks (Technical Report)

We study the problem of computing a minimal subset of nodes of a given asynchronous Boolean network that need to be controlled to drive its dynamics from an initial steady state (or attractor) to a target steady state. Due to the phenomenon of state-space explosion, a simple global approach that performs computations on the entire network, may not scale well for large networks. We believe that efficient algorithms for such networks must exploit the structure of the networks together with their dynamics. Taking such an approach, we derive a decomposition-based solution to the minimal control problem which can be significantly faster than the existing approaches on large networks. We apply our solution to both real-life biological networks and randomly generated networks, demonstrating promising results.

==> Discussion.tex <==
%!TEX root = ms.tex

As mentioned in the introduction, the problem of minimal control is PSPACE-hard and efficient algorithms are unlikely for the general case. Yet in retrospect, one might ask what is the inherent characteristic of our decomposition-based approach that makes it so efficient compared with a standard brute-force approach for the real-life networks that we studied.  We put forward a couple of heuristics which we believe explains and crucially determines the success of our approach. Our method exploits the structure of the underlying network , that is, if the structure of the network satisfies certain heuristics, our method would be fairly efficient. One such heuristic is that the basins of attraction computed at each step is small compared with the total number of states in the transition system. This cuts down the state space that needs to be considered in every subsequent step thus improving efficiency.
%

Another heuristic is that the number of blocks is small compared with the total number of nodes in the network. Otherwise, the method has to compute a large number of local transition systems (as many as the number of blocks) which hampers its efficiency.
%
However, the number of blocks in the network cannot be too few either. Otherwise, our approach comes close to the brute-force approach in terms of efficiency. Note that if the entire network is one single giant block, then our method is the same as the brute-force approach and there is no gain in efficiency. One might thus conjecture that there is an optimal block-to-node ratio, given which, our decomposition-based method fares the best.
%




